A Formal Proof of the Irrationality of $\zeta(3)$

This paper presents a complete formal verification of a proof that the evaluation of the Riemann zeta function at 3 is irrational, using the Coq proof assistant. This result was first presented by Ap\'ery in 1978, and the proof we have formalized essentially follows the path of his original presentation. The crux of this proof is to establish that some sequences satisfy a common recurrence. We formally prove this result by an a posteriori verification of calculations performed by computer algebra algorithms in a Maple session. The rest of the proof combines arithmetical ingredients and asymptotic analysis, which we conduct by extending the Mathematical Components libraries.

==> defManSSR.tex <==
%=======================================================================
% A listing mode for ssr Gallina (Assia Mahboubi 2007)

\lstdefinelanguage{SSR} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside},

% Gallina
morekeywords=[2]{forall, exists, exists2, fun, fix, cofix, struct,
      match, with, end, as, in, return, let, if, is, then, else,
      for, nosimpl},
% 'of' is removed from this list as it occurs in comments.

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{
         pose, set, move, case, elim, apply, clear,
            hnf, intro, intros, generalize, rename, pattern, after,
            destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr, vm_compute,
         symmetry, transitivity, auto, split, left, right,
         autorewrite, lia, intlia},

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
 literate=
        {->}{{$\rightarrow\ $}}2
%       {->}{{\tt ->}}3
%	{<-}{{$\leftarrow\,$}}2
%       {<-}{{\tt <-}}2
%       {>->}{{$\mapsto$}}3
        {<}{{$<\;\;$}}1
        {<=}{{$\leq\;\;$}}1
        {>=}{{$\geq\;\;$}}1
%       {<>}{{$\neq$}}1
        {/\\}{{$\wedge\;\;$}}2
        {\\/}{{$\vee\;\;$}}2
        {^~}{{\textvisiblespace$\;\;$}}2
        {~~}{{$\lnot\;\;$}}2
%       {<->}{{$\leftrightarrow\;$}}3
%       {<=>}{{$\Leftrightarrow\;$}}3
%       {:nat}{{$~\in\mathbb{N}$}}3
%	{fforall\ }{{$\forall_f\,$}}1
	{forall\ }{{$\forall\ \!$}}1
	{exists\ }{{$\exists\ \!$}}1
        {MAPLE}{{\raisebox{-0.8cm}[0cm][0cm]{\hspace{18mm}\includegraphics[width=1cm]{maple}}}}1
	{^2}{{$^2$}}1
	{^3}{{$^3$}}1
	{^4}{{$^4$}}1
	{^5}{{$^5$}}1
	{^6}{{$^6$}}1
%       {negb}{{$\neg$}}1
%       {spp}{{:*:\,}}1
%       {~}{{$\sim$}}1
%       {\\in}{{$\in\;$}}1
%       {/\\}{$\land\,$}1
%       {:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
%       {=>}{{\tt =>}}2
%       {:=}{{{\tt:=}\,\,}}2
%       {==}{{$\equiv$}\,}2
        {!=}{{$\neq$}\ }2
        {_cf0}{{$_{{0}}$}}1
        {_cf1}{{$_{{1}}$}}1
        {_cf2}{{$_{{2}}$}}1
        {_cf0_0}{{$_{{00}}$}}1
%        {_cf0}{{$_{\mbox{cf}_{0}}$}}1
%        {_cf1}{{$_{\mbox{cf}_{1}}$}}1
%        {_cf2}{{$_{\mbox{cf}_{2}}$}}1
%        {_cf0_0}{{$_{\mbox{cf}_{00}}$}}1
%       {^-1}{{$^{-1}$}}1
%       {elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2
,

% Comments delimiters, we do turn this off for the manual
%comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily\footnotesize,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{dkviolet}},

% Style for gallina keywords
keywordstyle=[2]{\ttfamily\color{dkgreen}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{lightblue}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
%commentstyle=\rmfamily,

}

